Noise Stability is computable and low dimensional

Questions of noise stability play an important role in hardness of approximation in computer science as well as in the theory of voting. In many applications, the goal is to find an optimizer of noise stability among all possible partitions of $\mathbb{R}^n$ for $n \geq 1$ to $k$ parts with given Gaussian measures $\mu_1,\ldots,\mu_k$. We call a partition $\epsilon$-optimal, if its noise stability is optimal up to an additive $\epsilon$. In this paper, we give an explicit, computable function $n(\epsilon)$ such that an $\epsilon$-optimal partition exists in $\mathbb{R}^{n(\epsilon)}$. This result has implications for the computability of certain problems in non-interactive simulation, which are addressed in a subsequent work.

==> communication.tex <==


\section{Application: Decidability of non-interactive correlation distillation}~\label{sec:application} 

In this section, we will sketch a proof of Lemma~\ref{lem:projection}. As we have seen earlier, this Lemma suffices to prove Corollary~\ref{corr:decidability-2} for any finite $k$. Let us recall the statement of Lemma~\ref{lem:projection}
\begin{customlemma}{\ref{lem:projection}}
Given $\mathcal{A}$, $\mathcal{B}$ and $\bP$ and error parameter $\epsilon>0$, there exists $m_0 = m_0 (|\bP|, \epsilon)$ such that the following holds: for any $f: \mathcal{A}^n \rightarrow [k]$ and $g: \mathcal{B}^n \rightarrow [k]$, there exist $\tilde{f}: \mathcal{A}^{m_0} \rightarrow [k]$ and $\tilde{g}: \mathcal{B}^{m_0} \rightarrow [k]$ such that $\marg_1(\tilde{f}) = \marg_1(f)$, $\marg_2(\tilde{g}) = \marg_2(g)$ and 
$\mathsf{Corr}(\tilde{f}, \tilde{g}) \ge \mathsf{Corr}(f,g) -\epsilon$. Further, given $\marg_1(f)$, $\marg_2(g)$ and $\mathsf{Corr}(f,g)$, there is an algorithm which runs in time $O_{|\bP|, \epsilon}(1)$ and outputs $\tilde{f}$ and $\tilde{g}$ satisfying the aforementioned guarantee. 
\end{customlemma}

We will only give a sketch of the proof of this lemma. In fact, we will prove the ``seemingly  weaker" version in the sense that we will show how to construct
$\tilde{f}$ and $\tilde{g}$ such that $|\marg_1(\tilde{f}) - \marg_1(f) |, |\marg_2(\tilde{g}) - \marg_2(g) | \le \epsilon$ and $\mathsf{Corr}(\tilde{f}, \tilde{g}) \ge \mathsf{Corr}(f, g) - \epsilon$. However, as we have seen before, this distinction is irrelevant as in given such a $\tilde{f}$ and $\tilde{g}$ with approximately correct marginals (up to error $\epsilon$), it is easy to construct one with exactly correct marginals and the modification decreases $\mathsf{Corr}(\tilde{f}, \tilde{g})$ by at most $\epsilon$. 

Similar to Ghazi \emph{et~al.}~\cite{GKS:16}, we can reduce the proof of this lemma to the $\mathsf{Gaussian}(\rho)$ case (for some $\rho>0$).  
Recall, by $\mathsf{Gaussian}(\rho)$ case, we mean $\mathcal{A} = \mathcal{B}= \mathbb{R}$ and $\bP= (\bX, \bY)$ be $2$-dimensional jointly Gaussian random variable where each marginal is a standard normal and their correlation is $\rho$. 
The reduction  to the $\mathsf{Gaussian}(\rho)$ case  follows the steps of Ghazi \emph{et~al.} and uses standard Boolean function analysis machinery. We will describe these steps and indicate what, if any, changes need to be made. Once we are in the Gaussian case, we will appeal to (a slight generalization of) Theorem~\ref{thm:main-stab}:


\begin{comment}
 we will sketch a proof of the following theorem.  
\begin{theorem}~\label{thm:decidability-k}
For any finite $k$, given probability spaces $(\mathcal{A} \times \mathcal{B}, \bP)$, there is 
an algorithm running in time $O_{|(\mathcal{A} \times \mathcal{B}, \bP)|, \delta}(1)$ such that given $\boldsymbol{\mu} = (\mu_1, \ldots, \mu_k)$ and $\boldsymbol{\nu}=(\nu_1, \ldots, \nu_k)$ (where $\boldsymbol{\mu}, \boldsymbol{\nu} \in \Delta_k$) and parameter $\kappa \in [0,1]$, it distinguishes between the following two cases: 
\begin{enumerate}
\item There exists $n \in \mathbb{N}$ and $f: \mathcal{A}^n \rightarrow [k]$ and $g: \mathcal{B}^n \rightarrow [k]$ such that for $(\bX,\bY) \sim \bP$, if $\bQ = (f(\bX^n), g(\bY^n))$, 
then (i) For $1 \le j \le k$, $\sum_{\ell=1}^k \bQ(j, \ell) = \mu_j$ and $\sum_{\ell=1}^k \bQ(\ell, j) = \nu_j$, (ii) 
$|\sum_{\ell=1}^k \bQ(\ell, \ell) - \kappa| \le 3\delta$.  In this case, there is an explicit $n_0 = n_0(|(\mathcal{A} \times \mathcal{B}, \bP)|, \delta)$ such that $f: \mathcal{A}^{n_0} \rightarrow [k]$ and $g: \mathcal{B}^{n_0} \rightarrow [k]$. Further, the functions $f$ and $g$ are explicitly computed. 
\item For any $n \in \mathbb{N}$ and $f: \mathcal{A}^n \rightarrow [k]$ and $g: \mathcal{B}^n \rightarrow [k]$ such that for $(\bX,\bY) \sim \bP$,  if $\bQ = (f(\bX^n), g(\bY^n))$, (i) For $1 \le j \le k$, $\sum_{\ell=1}^k \bQ(j, \ell) = \mu_j$ and $\sum_{\ell=1}^k \bQ(\ell, j) = \nu_j$, then  
$|\sum_{\ell=1}^k \bQ(\ell, \ell) - \kappa| > 10\delta$.
\end{enumerate}
\end{theorem}


We will not give a complete proof of this theorem but instead just give a sketch of this theorem as several of the steps in the proof closely resemble the proof of Corollary~\ref{corr:decidability-2} from \cite{GKS:16}. Note that to prove Theorem~\ref{thm:decidability-k}, it suffices to prove the following lemma. 
\begin{lemma}~\label{lem:comm-redn}
Given probability space $(\mathcal{A} \times \mathcal{B}, \bP)$ and functions $f: \mathcal{A}^n \rightarrow [k]$ and $g: \mathcal{B}^n \rightarrow [k]$ for any $\delta>0$, there exists 
an explicit $n_0 = n_0(|(\mathcal{A} \times \mathcal{B}, \bP)|, \delta)$ such that $\tilde{f}: \mathcal{A}^{n_0} \rightarrow [k]$ and $\tilde{g}: \mathcal{B}^{n_0} \rightarrow [k]$ with the following property: Let $\bQ = (f(\bX^n), g(\bY^n))$ and $\tilde{\bQ} = (\tilde{f}(\bX^{n_0}), \tilde{g}(\bY^{n_0}))$. Then,  (i) For $1 \le j \le k$, $|\sum_{\ell=1}^k \bQ(j, \ell) - \tilde{\bQ}(j, \ell)| \le \delta$ and $|\sum_{\ell=1}^k \bQ( \ell,j) - \tilde{\bQ}(\ell,j)| \le \delta$
and (ii) $\mathsf{Corr}(\bQ) - \mathsf{Corr}(\tilde{\bQ}) \le \delta$. 
\end{lemma}
\end{comment}
\begin{lemma}~\label{lem:two-reduction}
Let $f,g: \mathbb{R}^n \rightarrow [k]$. Then, for any     
  $t>0$ and $\epsilon>0$, there exists explicitly computable $n_0= n_0(\epsilon,k)$ and $d = d(\epsilon,k)$ and functions 
$\tilde{f}, \tilde{g}: \mathbb{R}^{n_0} \rightarrow [k]$ which are degree-$d$ PTFs such that \begin{enumerate}
\item $\Vert \mathbf{E}[f] - \mathbf{E} [\tilde{f}] \Vert_1 \le \epsilon$,  $\Vert \mathbf{E}[g] - \mathbf{E} [\tilde{g}] \Vert_1 \le \epsilon$. 
\item $\langle \tilde{f}, P_t \tilde{g} \rangle  \ge \langle f, P_t g \rangle - \epsilon$. 
\end{enumerate}
In the above, all expectations and probabilities are taken with respect to the standard Gaussian measure on the relevant dimensions. 
\end{lemma}
The difference between Lemma~\ref{lem:two-reduction} and Theorem~\ref{thm:main-stab} is that there are now two functions
instead of one. However, its proof (we will give only a sketch here) follows from the same machinery that we used to prove
Theorem~\ref{thm:main-stab}.
To prove a two-function version of Lemma~\ref{lem:1}, we first apply the ``rounding arguments'' to $P_t g$, producing
a function $f'$ with bounded Hermite tails, $\E[f'] = \E[f]$, and $\inr{f'}{P_t g} \ge \inr{f}{P_t g} - \epsilon/2$.
Then we apply the rounding argument again to $P_t \tilde f$, to produce a function $\tilde g$ with bounded Hermite
tails, $\E[g'] = \E[g]$, and $\inr{P_t f'}{g'} \ge \inr{P_t f'}{g} - \epsilon/2$.
Putting these two steps (and the fact that $P_t$ is self-adjoint) together, we have
$\inr{f'}{P_t g'} \ge \inr{f}{P_t g} - \epsilon$. This proves the two-function version of Lemma~\ref{lem:1}, and we
can apply Lemma~\ref{lem:2} to $f'$ and $g'$ individually, thereby turning $f'$ and $g'$ into bounded-degree PTFs.

Having obtained these PTFs, one can reduce the number of variables to $n_0 = n_0 (k,\epsilon)$ by adapting the machinery of Theorem~\ref{thm:reduction}. Again, while one cannot reduce the number of variables in $f'$ and $g'$ to $n_0$ by directly appealing as a black-box to Theorem~\ref{thm:reduction}, it is easy to show that if one applies Theorem~\ref{thm:reduction} to $f'$ (resp. $g'$) to obtain $\tilde{f}$ (resp. $\tilde{g}$), then $\langle \tilde{f} , P_t \tilde{g} \rangle\ge \langle f' , P_t g' \rangle - \epsilon/2$. 

We now focus on using Lemma~\ref{lem:two-reduction} to 
prove Lemma~\ref{lem:projection}. To do this, we will have to briefly recall the notion of ``Fourier analysis over general product spaces" (see Mossel~\cite{Mossel:10} for a reference). We now do a brief interlude to describe the basics of this machinery. 



%The proof will first identify every element in $i \in [k]$ with the standard unit vector $\mathbf{e}_i$ in $\mathbb{R}^k$. Thus, we now seek to find $f: \mathcal{A}^n \rightarrow \mathbf{E}_k$ and $g: \mathcal{B}^n \rightarrow \mathbf{E}_k$ such that $\mathbf{E}[f(\bX^n) ] = \boldsymbol{\mu}$, $\mathbf{E}[g(\bY^n)] = \boldsymbol{\nu}$ and maximize $\mathbf{E}[\langle f(\bX^n) , g(\bY^n) \rangle]$. Instead of considering functions $f$ and $g$, we will allow ourselves to consider functions with range $\Delta_k$ instead with the same requirement. This is because of the following basic ``rounding strategy" described below. 
%~\\
%\textbf{Rounding strategy: } Given $z \in \Delta_k$, the \emph{natural rounding strategy} first partition the unit interval $[0,1]$ into $k$ intervals of size $z_1, \ldots, z_k$. Then, sample $r$ uniformly from $[0,1]$ and output $i \in [k]$ depending on the interval in which $r$ falls. 
%~\\
%Now, note that given any functions $f$ and $g$ with range $\Delta_k$, if Alice and Bob apply independent rounding strategies on the outputs of $f$ and $g$, then (i) their outputs are now in $\mathbf{E}_k$, (ii) probability that Alice(resp. Bob) outputs $i$ is $\mu_i$ (resp. $\nu_i$), (iii) 
%probability that Alice and Bob have the same output is $\mathbf{E}[\langle f(\bX^n) , g(\bY^n) \rangle]$.
%~\\
%Thus, without loss of generality, if we are in Case (1) of Theorem~\ref{thm:decidability-k}, we can output $f$ and $g$ with range $\Delta_k$. To sketch  the proof of Theorem~\ref{thm:decidability-k}, we need to recall some basics of Fourier analysis over product spaces. See ~\cite{Mossel:10} for more details. We now do a brief interlude for Fourier analysis over product spaces. 
\subsection{Fourier analysis over product spaces} 
To do this, we need to first understand the structure of the probability space $\bP$ defined on $\mathcal{A} \times \mathcal{B}$.  Without loss of generality, we can assume $\mathcal{A}= \mathcal{B}= [m]$. Let the marginal of $\bP$ on $\mathcal{A}$ be $\bP_{\mathcal{A}}$ and that 
on $\mathcal{B}$ be  $\bP_{\mathcal{B}}$.
Given functions $f : \mathcal{A} \rightarrow \mathbb{R}$ and $g: \mathcal{B} \rightarrow \mathbb{R}$ and $(\bX, \bY) \sim P$, 
we let $\mathsf{Cov} [f,g]$ denote the covariance of the pair $f( \bX )$ and $g( \bY )$. Likewise, $\mathsf{Var}(f)$ denotes the variance of $f( \bX )$ and $\mathsf{Var}(g)$ denotes the variance of $g( \bY )$.
Further, for any domain $\mathcal{X}$, we will let $\mathbf{1}$ denote the function which maps every point to $1$. Define
\begin{equation}~\label{eq:rho-def}
\rho = \sup_{{f: \mathcal{A} \rightarrow \mathbb{R}, g: \mathcal{B} \rightarrow \mathbb{R} } } \bigg\{ \mathsf{Cov}(f,g) : \mathsf{Var}(f) = \mathsf{Var}(g)=1 \bigg\}.
\end{equation}
 Then, Mossel~\cite{Mossel:10} shows that one can construct a sequence of functions  $\{\mathcal{X}_j\}_{j=0}^{m-1}$ and  $\{\mathcal{Y}_j\}_{j=0}^{m-1}$ such that $\mathcal{X}_j : \mathcal{A}\rightarrow \mathbb{R}$, $\mathcal{Y}_j: \mathcal{B} \rightarrow \mathbb{R}$ which have the following properties. Note that we will be equivalently thinking of $\mathcal{X}_j$, $\mathcal{Y}_j$ as random variables where the underlying measure on $\mathcal{A} \times \mathcal{B}$ is given by $\bP$. 
\begin{enumerate}
\item Both $\mathcal{X}_0$ and $\mathcal{Y}_0$ are the identically one function $\mathbf{1}$ (for the respective domains). 
\item $\mathbf{E}[\mathcal{X}_i (\bX) \cdot \mathcal{X}_j (\bX) ] = \mathbf{E}[\mathcal{Y}_i (\bY) \cdot \mathcal{Y}_j (\bY)]= \delta_{i=j}$ i.e. the sequence $(\mathcal{X}_0, \ldots, \mathcal{X}_{m-1})$ and  $(\mathcal{Y}_0, \ldots, \mathcal{Y}_{m-1})$ are an orthonormal basis. 
\item $\mathbf{E}[\mathcal{X}_i (\bX) \cdot \mathcal{Y}_j (\bY) ] =0$ if $i \not =j$. 
\item $\mathbf{E}[\mathcal{X}_i (\bX) \cdot \mathcal{Y}_i (\bY) ] =\rho_i$ for some $\rho_i \in [0,1]$ with $1=\rho_0 \ge \rho_1 \ge \ldots \ge \rho_{m-1}$ and $\rho_1 = \rho$.
\end{enumerate}

Having constructed this basis, we can now construct a basis for the space $\mathcal{A}^n \times \mathcal{B}^n$ endowed with the measure $\bP^n$ as follows: For $\bs{\sigma}= (\sigma_1, \ldots, \sigma_n) \in \mathbb{Z}_m^n$, we define $\mathcal{X}_{\bs{\sigma}}: \mathcal{A}^n \rightarrow \mathbb{R}$ and
$\mathcal{Y}_{\bs{\sigma}}: \mathcal{B}^n \rightarrow \mathbb{R}$ as 
$$
\mathcal{X}_{\bs{\sigma}} (x_1, \ldots, x_n) = \prod_{i=1}^n \mathcal{X}_{\sigma_i}(x_i), \ \ \mathcal{Y}_{\bs{\sigma}} (y_1, \ldots, y_n) = \prod_{i=1}^n \mathcal{Y}_{\sigma_i}(y_i), 
$$
where $(x_1, \ldots, x_n) \in \mathcal{A}^n$ and $(y_1, \ldots, y_n) \in \mathcal{B}^n$. It is easy to see that this defines an orthonormal basis for the space of functions $\mathcal{A}^n$ (resp. $\mathcal{B}^n$).  Now, note that every $f : \mathcal{A}^n \rightarrow \mathbb{R}^k$ and  $g : \mathcal{B}^n \rightarrow \mathbb{R}^k$ can be expressed as
\[
f(x) = \sum_{\bs{\sigma}} \widehat{f}(\bs{\sigma}) \mathcal{X}_{\bs{\sigma}}(x) , \ \ g(y) = \sum_{\bs{\sigma}} \widehat{g}(\bs{\sigma}) \mathcal{Y}_{\bs{\sigma}}(y). 
\]
Here $\widehat{f}(\bs{\sigma}) , \widehat{g}(\bs{\sigma}) \in \mathbb{R}^k$. All the expectations below are on $(\mathcal{A}^n, \mathcal{B}^n)$ endowed with the measure $\bP^n$. 


From the definition, it is not hard to prove the following elementary relations.  We refer the reader to \cite{Mossel:10} for more details. Also, let $\mathbf{0} = (0, \ldots, 0) \in \mathbb{Z}^n$.  
\begin{eqnarray*}
\mathbf{E} [f] = \widehat{f}(\mathbf{0}), \ \mathbf{E}[\langle f, f \rangle]= \sum_{\bs{\sigma}} \langle \widehat{f}(\bs{\sigma}),  \widehat{f}(\bs{\sigma}) \rangle\ \ \  \mathbf{E}[\langle f, g \rangle] = \sum_{\bs{\sigma}} \langle \widehat{f}(\bs{\sigma}) ,\widehat{g}(\bs{\sigma}) \rangle \cdot \boldsymbol{\rho}^{\bs{\sigma}}.
\end{eqnarray*}
Here $\boldsymbol{\rho}^{\bs{\sigma}} = \prod_{i=1}^n \rho_{\sigma_i}$. 
For any $\bs{\sigma}$, $\mathsf{deg}(\bs{\sigma})$ is the number of non-zero coordinates in $\bs{\sigma}$. 
For any $f$ as defined above, we define $\mathsf{deg}(f) = \max_{\bs{\sigma} : \widehat{f}(\bs{\sigma}) \not =0} \mathsf{deg}(\bs{\sigma})$. 
To get an intuition for these quantities, one should think of expressing $f = \sum_{\bs{\sigma}} \widehat{f}(\bs{\sigma}) \mathcal{X}_{\bs{\sigma}}$ as the ``Fourier expansion" of $f$. In particular, the elements $\{\mathcal{X}_{\bs{\sigma}}\}$ form the ``Fourier basis". The last definition we require is that of influence. For any $i \in [n]$, $\mathsf{Inf}_i(f) = \sum_{\bs{\sigma}: \sigma_i \not =0} \Vert \widehat{f}(\bs{\sigma})\Vert_2^2$. With this, we describe the proof of Lemma~\ref{lem:projection}. 
%With this, we describe the steps in the proof of \cite{GKS:16}. Note that to prove Corollary~\ref{corr:decidability-2}, it suffices to show the following: 

\subsection{Proof of Lemma~\ref{lem:projection}}
%
%
%
% Namely, we start with the assumption that we are in Case (1) i.e. there exist $f: \mathcal{A}^n \rightarrow \Delta_2$ and $g: \mathcal{B}^n \rightarrow \Delta_2$ which satisfy 
Given error parameter $\epsilon>0$, let us choose a suitably small $\delta = \delta(\epsilon, k,\bP) >0$. The value $\delta$ shall be chosen to be sufficiently small so as to satisfy the requirements of all the lemmas that we will invoke to prove Lemma~\ref{lem:projection}. 


\begin{enumerate}
\item \emph{Smoothing of strategies:} Given any $\delta>0$, Lemma~6.2 from \cite{Mossel:10} shows  
 that there exists $f_{\delta}: \mathcal{A}^n \rightarrow \Delta_k$ and $g_{\delta}: \mathcal{B}^n \rightarrow \Delta_k$
 with the following properties: 
 (i) $\marg_1(f_{\delta}) = \marg_1(f)$ and $\marg_2(g_{\delta}) = \marg_2(g)$. (ii) There exists (an explicit function) $d' = d'(\delta, \rho)$ such that 
 $\sum_{|\bs{\sigma}| > d'} \Vert \widehat{f_\delta} (\bs{\sigma}) \Vert_2^2, \sum_{|\bs{\sigma}| > d'} \Vert \widehat{g_\delta} (\bs{\sigma}) \Vert_2^2 \leq \delta$. (iii) $\mathbf{E}[f_{\delta}(\bX^n) \cdot g_{\delta}(\bY^n)] \ge \mathbf{E}[f(\bX^n) \cdot g(\bY^n)]  - \delta$. The idea behind proving this lemma is to \emph{dampen both $f$ and $g$ with $\delta$-noise.}%
 This step is exactly the same as Lemma~4.5 from \cite{GKS:16}. 
\item \emph{Obtaining low-influence functions:} Note that the functions $f_{\delta}$ and $g_{\delta}$ are essentially (vector-valued) low-degree polynomials. Using arguments similar to the ``multidimensional" regularity lemma from \cite{DDS14} (Lemma~45 in that paper), one can show that $f_\delta$ and $g_\delta$ have low max-influence under random restrictions.
More precisely, there is a subset $H \subseteq [n]$ of size $h=h(d',\delta)$ with the following property: let $\mathcal{A}^n = \mathcal{A}^H \times \mathcal{A}^{[n] \setminus H}$, i.e. we split our input into the coordinates lying in $H$ and those lying outside $H$. Likewise, $\mathcal{B}^n = \mathcal{B}^H \times \mathcal{B}^{[n] \setminus H}$. Then, over random samplings $(x_H, y_H) \sim (\bX^H, \bY^H)$, with probability $1- \delta$, the functions $f_\delta(x_H, \cdot) : \mathcal{A}^{[n] \setminus H} \rightarrow \Delta_k$ and  $g_\delta(y_H, \cdot) : \mathcal{B}^{[n] \setminus H} \rightarrow \Delta_k$ have max-influence smaller than $\delta$.
This is again exactly the same as Lemma~5.1 from \cite{GKS:16}. In Lemma~5.1, \cite{GKS:16} use the regularity lemma from \cite{DSTW:10} as they are handling two polynomials.  Since we have to handle $k$-polynomials, one can use the more general version of the polynomial regularity lemma from \cite{DDS14}.  
%\item \emph{Obtaining low-influence functions: } In this step, \cite{GKS:16} show that given functions $f_{\delta}, g_{\delta}$ as above, it is possible to find a set $H \subseteq [n]$ of size $h=h(d,\delta)$ with the following property: Let $\mathcal{X}^n = \mathcal{X}^H \times \mathcal{X}^{[n] \setminus H}$ i.e. we split our input into the coordinates lying in $H$ and those lying outside $H$. Likewise, $\mathcal{Y}^n = \mathcal{Y}^H \times \mathcal{Y}^{[n] \setminus H}$. Then, using the regularity lemma for low-degree polynomials~\cite{DSTW:10}, the authors show that over random samplings $(x_H, y_H) \sim (\mathcal{X}^H, \mathcal{Y}^H)$, with probability $1- \delta$, the functions $f(x_H, \cdot) : \mathcal{A}^{[n] \setminus H} \rightarrow [0,1]$ and  $g(y_H, \cdot) : \mathcal{B}^{[n] \setminus H} \rightarrow [0,1]$ such that $\max \mathsf{Inf} (f(x_H, \cdot)), \max \mathsf{Inf}(g(y_H, \cdot)) \le \delta$. 
\item \emph{Low-influence correlation bounds:} 
This is the step where we use Lemma~\ref{lem:two-reduction}. To do this, consider any restriction $(x_H, y_H) \sim (\bX^H, \bY^H)$ such that $\max \mathsf{Inf} (f(x_H, \cdot)), \max \mathsf{Inf}(g(y_H, \cdot)) \le \delta$. By appealing to the invariance principle proven in \cite{Mossel:10} (which is an extension of the result of \cite{MOO10}), one can show the following: 
 Let $\{\underline{\mathcal{X}_{j}}\}_{0\le j \le m-1}, \{\underline{\mathcal{Y}_{j}}\}_{0\le j \le m-1}$ be jointly Gaussian random variables such that the pairwise correlations 
 of this family is precisely the same as $\{{\mathcal{X}_{j}}\}_{0\le j \le m-1}, \{{\mathcal{Y}_{j}}\}_{0\le j \le m-1}$. In other words, $\E[\ul{\mathcal{X}}_i \ul{\mathcal{X}}_j] = \E[\ul{\mathcal{Y}}_i \ul{\mathcal{Y}}_j] = \delta_{i=j}$
 and $\E[\ul{\mathcal{X}}_i \ul{\mathcal{Y}}_j] = \delta_{i=j} \rho_i$.
Let $\ul{\bX} = (\ul{\mathcal{X}}_1, \ldots, \ul{\mathcal{X}}_m)$ and $\ul{\bY} = (\ul{\mathcal{Y}}_1, \ldots, \ul{\mathcal{Y}}_m)$. {For simplicity of description, let us now assume that $\rho_1 = \ldots = \rho_{m-1} = \rho$. In our setting, since we just seek to maximize correlation, it is easy to get rid of this assumption and just set $\rho = \max_{1 \le i \le m-1} \rho_i$. However, to keep this discussion simple, we will just focus on $\rho_1 = \ldots = \rho_{m-1} = \rho$.}
The invariance principle from \cite{Mossel:10} shows that there is a function $\ul{f} : \mathcal{A}^H \times (\mathbb{R}^{m})^{[n] \setminus H} \rightarrow \Delta_k$ and $\ul{g}:  \mathcal{B}^H \times (\mathbb{R}^{m})^{[n] \setminus H} \rightarrow \Delta_k$ with the following properties: 
~\\
For every $(x_H, y_H) \sim (\bX^H, \bY^H)$, let $\ul{f}(x_H, \cdot): (\mathbb{R}^m)^{[n] \setminus H} \rightarrow \Delta_k$ and $\ul{g}(y_H, \cdot): (\mathbb{R}^m)^{[n] \setminus H} \rightarrow \Delta_k$ be the functions obtained by restricting the coordinates in $H$ in $\ul{f}$ (resp. $\ul{g}$) to $x_H$ (resp. $y_H$). Consider a pair $(x_H, y_H)$ such that 
 $\max \mathsf{Inf} (f(x_H, \cdot)), \max \mathsf{Inf}(g(y_H, \cdot)) \le \delta$. Then, 
\begin{eqnarray}
&&\Vert \mathbf{E}_{x_H \in \bX^H}[\ul{f}(x_H, \ul{\bX}^{[n] \setminus H})] - \mathbf{E}_{x_H \in \bX^H}[f(x_H, \bX^{[n] \setminus H})] \Vert_1 \le \delta. \label{eq:ab1}
\\
&&\Vert \mathbf{E}_{y_H \in \bY^H}[\ul{g}(y_H, \ul{\bY}^{[n] \setminus H})] - \mathbf{E}_{y_H \in \bY^H}[g(y_H, \bY^{[n] \setminus H})] \Vert_1 \le \delta. \nonumber \\
&&\mathop{\mathbf{E}}_{(x_H,y_H) \in (\bX^H,\bY^H)}[\langle \ul{f}(x_H, \ul{\bX}^{[n] \setminus H}),  \ul{g}(y_H, \ul{\bY}^{[n] \setminus H}) \rangle] \ge \mathop{\mathbf{E}}_{(x_H,y_H) \in (\bX^H,\bY^H)}[\mathsf{Corr}( {f}(x_H, \cdot), {g}(y_H, \cdot) )] - \delta, \nonumber
\end{eqnarray}
However, note that for any given $(x_H, y_H)$, the inputs to $\ul{f}(x_H, \cdot)$ and $\ul{g}(y_H, \cdot)$ 
are $\rho$-correlated Gaussians. Or, in other words, the left hand side of the last inequality is the same as
\[
\mathop{\mathbf{E}}_{(x_H,y_H) \in (\bX^H,\bY^H)}[\langle \ul{f}(x_H, \ul{\bX}^{[n] \setminus H}), P_t  \ul{g}(y_H, \ul{\bX}^{[n] \setminus H}) \rangle],
\]
where $t =\ln (1/\rho)$. 
However, now we can appeal to Lemma~\ref{lem:two-reduction} and we can assume that each of the functions $\ul{f}(x_H, \cdot)$ 
and $\ul{g}(x_H, \cdot)$ are degree $d = d(k,\epsilon)$ PTFs over $n_0 = n_0(k,\epsilon)$ variables (where both $d$ and $n_0$ are explicitly computable).  Note that the functions $\ul{f}(x_H, \cdot)$ and $\ul{g}(y_H,\cdot)$ are $\Delta_k$ valued as opposed to $[k]$-valued. However, it is easy to see that given a $\Delta_k$ valued function with some noise stability and measure, it is possible to get a $[k]$-valued function with the same measure and noise stability (see~\cite{IsakssonMossel:12} for such an argument).  We do not give the argument here. 
Let us define $(\bZ_1, \bZ_2)$ to be two standard $\rho$-correlated Gaussians. Note that $(\ul{\bX}, \ul{\bY})$ are $m$ independent identical copies of $(\bZ_1, \bZ_2)$. With this notation and assuming that $\ul{f}(x_H, \cdot)$ and $\ul{g}(y_H, \cdot)$ are over $n_0$ coordinates, 
 we can now rewrite the equations in (\ref{eq:ab1}) as
   \begin{eqnarray}
&&\Vert \mathbf{E}_{x_H \in \bX^H}[\ul{f}(x_H, \bZ_1^{n_0})] - \mathbf{E}_{x_H \in \bX^H}[f(x_H, \bX^{[n] \setminus H})] \Vert_1 \le \delta. \label{eq:ab2}
\\
&&\Vert \mathbf{E}_{y_H \in \bY^H}[\ul{g}(y_H, \bZ_2^{n_0})] - \mathbf{E}_{y_H \in \bY^H}[g(y_H, \bY^{[n] \setminus H})] \Vert_1 \le \delta. \nonumber \\
&&\mathop{\mathbf{E}}_{(x_H,y_H) \in (\bX^H,\bY^H)}[\langle \ul{f}(x_H, \bZ_1^{n_0}),  \ul{g}(y_H, \bZ_2^{n_0}) \rangle] \ge \mathop{\mathbf{E}}_{(x_H,y_H) \in (\bX^H,\bY^H)}[\mathsf{Corr}( {f}(x_H, \cdot), {g}(y_H, \cdot) )] - \delta, \nonumber
\end{eqnarray}

 \item Note that after the last step, we obtain functions $\ul{f}$ and $\ul{g}$ which are over $n_0 + |H|$ coordinates where the first $H$ coordinates are in $\mathcal{A}$ (resp. $\mathcal{B}$) whereas the last $n_0$ coordinates are in $\mathbb{R}$. We  have almost accomplished what we set out to achieve. Namely, $\ul{f}$ and $\ul{g}$ are explicit functions on just $n_0 + |H|$ coordinates where $n_0 + |H| = O_{\epsilon, k, \bP}(1)$. 
 The problem is that
 the last $n_0$ coordinates for both $\ul{f}$ and $\ul{g}$ are in $\mathbb{R}$. 
  Further, given any $|H| < i \le n_0 + |H|$, the $i^{th}$ coordinate of $\ul{f}$ and $\ul{g}$ are distributed as 
  $\rho$-correlated standard Gaussians. To remedy both these problems at once, let us choose a value of $\ell$ (which will be fixed later). Define $m_0 = |H| + n_0 \cdot \ell$. Note that using (\ref{eq:rho-def}), the functions $\mathcal{X}_1$ and $\mathcal{Y}_1$ satisfy  
 \[
 \mathbf{E}_{\bX} [\mathcal{X}_1(\bX)]=  \mathbf{E}_{\bY} [\mathcal{Y}_1(\bY)] =0. \quad \mathbf{E}_{\bX} [\mathcal{X}_1^2(\bX)]=  \mathbf{E}_{\bY} [\mathcal{Y}_1^2(\bY)] =1. \quad \mathbf{E}_{(\bX,\bY)} [\mathcal{X}_1(\bX) \cdot \mathcal{Y}_1(\bY)]=\rho.
 \]
 We now define $\tilde{f}: \mathcal{A}^{m_0} \rightarrow [k]$ and $\tilde{g}: \mathcal{B}^{m_0} \rightarrow [k]$ as follows. Let the first $|H|$ coordinates of $m_0$ be indexed by $H$ and the rest $n_0 \cdot \ell$ coordinates be divided into $n_0$ blocks of size $\ell$ each. Now, let the variables to $\tilde{f}$ be denoted by $\{x_{i,j}\}_{1 \le i \le n_0, 1\leq j \le \ell}$  and the variables to $\tilde{g}$ be denoted by $\{y_{i,j}\}_{1 \le i \le n_0, 1\leq j \le \ell}$. We then define $\tilde{f}$ and $\tilde{g}$ as follows: 
 \[
 \tilde{f}(x_H, \{x_{i,j}\}) = \ul{f}\left( x_H, \frac{\mathcal{X}_1( x_{1,1}) +\ldots + \mathcal{X}_1(x_{1,\ell})}{\sqrt{\ell}},  \ldots, \frac{\mathcal{X}_1(x_{n_0,1}) +\ldots + \mathcal{X}_1(x_{n_0,\ell})}{\sqrt{\ell}}  \right)
 \]
 \[
 \tilde{g}(y_H, \{y_{i,j}\}) = \ul{g}\left( y_H, \frac{\mathcal{Y}_1( y_{1,1}) +\ldots + \mathcal{Y}_1(y_{1,m})}{\sqrt{m}},  \ldots, \frac{\mathcal{Y}_1(y_{n_0,1}) +\ldots + \mathcal{Y}_1(y_{n_0,m})}{\sqrt{m}}  \right)
 \]
 The intuition behind this construction is that for each of the last $n_0$ arguments to $\ul{f}$ and $\ul{g}$ (in the above definition), the induced distribution (using the central limit theorem) converges to the  distribution $(\bZ_1, \bZ_2)$. 
 To get the actual result, we can again apply to the invariance principle of Mossel~\cite{Mossel:10}. Namely. note that for any $x_H$, $\max_{i,j} \mathsf{Inf}_{i,j}(\tilde{f}(x_H, \cdot)) = \frac{1}{\sqrt{\ell}}$. Likewise, $\max_{i,j} \mathsf{Inf}_{i,j}(\tilde{g}(y_H, \cdot)) = \frac{1}{\sqrt{\ell}}$. Here $\mathsf{Inf}_{i,j} \tilde{f}(x_H, \cdot)$ denotes the influence of variable $x_{i,j}$ in the function $\tilde{f}(x_H, \cdot)$. 
Likewise,  $\mathsf{Inf}_{i,j} \tilde{g}(y_H, \cdot)$ denotes the influence of variable $y_{i,j}$ in the function $\tilde{g}(y_H, \cdot)$. Assume that each $(x_{i,j} , y_{i,j})$ is sampled as an i.i.d. copy of $(\bX,\bY)$. 
By choosing $\ell$ to be sufficiently large as a function of $\delta$, the invariance principle of Mossel~\cite{Mossel:10} implies that for every $(x_H, y_H) \sim (\bX^H, \bY^H)$
\[
\Vert \marg_1(\tilde{f}(x_H, \cdot)) -\mathbf{E}[\ul{f}(x_H, \bZ_1^{n_0})] \Vert_1 \le \delta.
\]
\[
\Vert \marg_2(\tilde{g}(y_H, \cdot)) -\mathbf{E}[\ul{g}(y_H, \bZ_2^{n_0})] \Vert_1 \le \delta.
\]
\[
\big| \mathsf{Corr}(\tilde{f} (x_H, \cdot), \tilde{g}(y_H,\cdot)) - \mathbf{E}[\langle \ul{f}(x_H, \bZ_1^{n_0}) , \ul{g}(y_H, \bZ_2^{n_0}) \rangle] \big| \le \delta. 
\]
Combining this with (\ref{eq:ab2}), we obtain that 
\[
\Vert \marg_1(\tilde{f})  -\marg_1({f}) \Vert_1 \le 2\delta. 
\]
\[
\Vert \marg_2(\tilde{g})  -\marg_2({g}) \Vert_1 \le 2\delta.
\]
\[
\mathsf{Corr}(\tilde{f}, \tilde{g}) - \mathsf{Corr}(f,g) \ge - 2\delta. 
\]
As long as we choose $\delta \le \epsilon/2$, this satisfies the requirements of Lemma~\ref{lem:projection}. Note that fixing $\delta$ fixes $\ell$ and thus fixes $m_0$. This finishes the proof.
\end{enumerate}


%$f_{\mathcal

 
 
% More precisely, the standard two dimensional central limit theorem implies the following: 
% \begin{theorem}~\cite{Feller}
% Let us define $\bW_1$ and $\bW_2$ as follows: 
% \[\bW_1 = \frac{f_{\mathcal{A}}(\bX_1) + \ldots + f_{\mathcal{A}}(\bX_m)}{\sqrt{m}} \ \  \  \bW_2 = \frac{f_{\mathcal{B}}(\bY_1) + \ldots + f_{\mathcal{B}}(\bY_m)}{\sqrt{m}}\]
% Here $(\bX_i, \bY_i)$ are independent copies of the random variable $(\bX,\bY)$. 
% Then, for any set $(\alpha_1, \alpha_2) \in \mathbb{R}^2$, 
% \[
% \big| \Pr[\bW_1 \le \alpha_1 \wedge \bW_2 \le \alpha_2] - \Pr[\bZ_1 \le \alpha_1 \wedge \bZ_2 \le \alpha_2] \big| \le O_{\bX,\bY}(1) \cdot (1/\sqrt{m}). 
% \]
% \end{theorem}
% 
 
% Further, to simulate the desired statistical behavior, we need the last $n_0$ coordinates of $\ul{f}$ (resp. $\ul{g}$) to be endowed with the distribution $\bZ_1$ (resp. $\bZ_2$) where $(\bZ_1, \bZ_2)$ are $\rho$-correlated standard Gaussians. To simulate $\rho$-correlated Gaussians given access to $\bP$, note that if $\bP= (\bX, \bY)$, then by definition, there exists functions 
% $f_{\mathcal{A}} : \mathcal{A} \rightarrow \mathbb{R}$ 
% and $g_{\mathcal{B}} : \mathcal{B} \rightarrow \mathbb{R}$ such that for any $\kappa$, $\exists m$ where $m = m(\kappa, \bP)$ such that for $\bW_1$ and $\bW_2$ defined as
% $$
% \bW_1 = \frac{f_{\mathcal{A}}(\bX_1) + \ldots + f_{\mathcal{A}}(\bX_m)}{\sqrt{m}} \ \  \  \bW_2 = \frac{f_{\mathcal{B}}(\bY_1) + \ldots + f_{\mathcal{B}}(\bY_m)}{\sqrt{m}}, 
% $$ 
% the distribution $(\bW_1, \bW_2)$ is $\kappa$-close to $(\bZ_1, \bZ_2)$ in Kolmogorov distance. This is a consequence of the central limit theorem. Here $(\bX_i, \bY_i)$ are independent copies of $\bP= (\bX, \bY)$. 
% 
% Set \new{$\kappa = \frac{\epsilon}{n_0^d}$} and let $m = m (\kappa, \bP)$ be the resulting value of $m$. Let us define $m_0 = |H| + n_0 \cdot m$ and define $\tilde{f}: \mathcal{A}^{ m_0} \rightarrow [k]$ and $\tilde{g}: \mathcal{B}^{ m_0 }\rightarrow [k]$ as follows: 
% Let the first $H$ coordinates of $\tilde{f}$ be denoted by $x_H$. For the other $n_0 \cdot m$ coordinates, break it into $n_0$ chunks of size $m$ each. Each such variable is denoted by $x_{i,j}$ where $1 \le i \le n_0$ and $1 \le j \le m$. Then, we define
% \[
% \tilde{f}(x_H, \{x_{i,j}\}) = \ul{f}\left( x_H, \frac{f_{\mathcal{A}}( x_{1,1}) +\ldots + f_{\mathcal{A}}(x_{1,m})}{\sqrt{m}},  \ldots, \frac{f_{\mathcal{A}}(x_{n_0,1}) +\ldots + f_{\mathcal{A}}(x_{n_0,m})}{\sqrt{m}}  \right)
% \]
% \[
% \tilde{g}(y_H, \{y_{i,j}\}) = \ul{g}\left( y_H, \frac{g_{\mathcal{B}}( y_{1,1}) +\ldots + g_{\mathcal{B}}(y_{1,m})}{\sqrt{m}},  \ldots, \frac{g_{\mathcal{B}}(y_{n_0,1}) +\ldots + g_{\mathcal{B}}(y_{n_0,m})}{\sqrt{m}}  \right)
% \]
% By appealing to the central limit theorem, we obtain that 
% \[
% \Vert \marg_1(\tilde{f})  - \mathbf{E}[\ul{f} ]  \Vert_1 \le \epsilon. 
% \]
%  \[
% \Vert \marg_2(\tilde{g})  - \mathbf{E}[\ul{g} ]  \Vert_1 \le \epsilon. 
% \]
% \[
% \mathsf{Corr}(\tilde{f}, \tilde{g}) - \mathbf{E}_{(x_H, y_H) \sim (\bX^H, \bY^H)} [\langle \ul{f}(x_H, \cdot) , P_t \ul{g}(y_H, \cdot) \rangle] \ge -\epsilon. 
% \]
% This finishes the proof of construction. 
%\end{itemize}
%%By appealing to Lemma~\ref{lem:two-reduction}, we get that every function $\ul{f}(x_H, \cdot)$ and $\ul{g}(y_H, \cdot)$ is a degree $d = d(\epsilon,k)$ PTF over $n_0 = n_0(k, \epsilon)$ variables. Note that while application of Lemma~\ref{lem:two-reduction} requires every coordinate of $\ul{\bX}$ to have precisely the same correlation, as we seek to maximize correlation, it suffices to restrict attention to $\ul{f}$ such that it is a function of only those coordinates where the corresponding correlation of the coordinates of $\ul{\bX}$ and $\ul{\bY}$ is precisely $\rho_1$. 
%%
%%
%%We can now appeal to Theorem~\ref{lem:two-reduction} to note that it suffices to choose $\ul{f}$ and $\ul{g}$ which are only functions of $n_0$ coordinates and are PTFs of degree $d= d(k,\epsilon)$. 





